Collapsing molecular clouds with tracer particles: Part II, Collapse Histories

In order to develop a complete theory of star formation, one essentially needs to know two things: what collapses, and how long it takes. This is the second paper in a series, where we query how long a parcel of gas takes to collapse and the process it undergoes. We embed pseudo-Lagrangian tracer particles in simulations of collapsing molecular clouds, identify the particles that end in dense knots, and then examine the collapse history of the gas. We find a nearly universal behavior of cruise-then-collapse, wherein a core stays at intermediate densities for a significant fraction of its life before finally collapsing. We identify time immediately before each core collapses, $t_{\rm{sing}}$, and examine how it transitions to high density. We find that the time to collapse is uniformly distributed between $0.25 t_{\rm{ff}}$ and the end of the simulation at $\sim 1 t_{\rm{ff}}$, and that the duration of collapse is universally short, $\Delta t \sim 0.1 t_{\rm{ff}}$, where $t_{\rm{ff}}$ is the free-fall time at the mean density. We describe the collapse in three stages; collection, hardening, and singularity. Collection sweeps low density gas into moderate density. Hardening brings kinetic and gravitational energies into quasi-equipartition. Singularity is the free-fall collapse, forming an envelope in rough energy balance and central over density in $\sim 0.1 t_{\rm{ff}}$.

==> REPORT1.tex <==
DONT TOUCH

Scientific Editor: Prof Andrew King

Assistant Editor's Comments:
Please ensure that all textual labels in figures are at least as large as the caption text; any smaller and they become too difficult to read. 


Reviewer's Comments:
Reviewer: Dr Mordecai-Mark Mac Low

Comments to the Author
This paper presents a study of the origins and evolution of cores forming in magnetized, turbulent, self-gravitating, isothermal gas.  The novelty of the study consists primarily in following the gas that eventually forms the cores using tracer particles originally uniformly distributed throughout the periodic domain.

I have several concerns about the numerical approximations used, and a number of more minor issues with the presentation that should also be corrected prior to recommending publication.

The biggest issues have to do with numerical resolution of turbulence and collapse:  

2.) 
* First, at the beginning of the run, a rather well-resolved model with 1024^3 zones is downsampled by an order of magnitude in linear resolution to 128^3 prior to turning on self-gravity.  The result of this downsampling, as emphasized by Seifried, Walch et al. (2017), is to erase the high-wavenumber end of the turbulent power spectrum.  The subsequent collapse and refinement has to be treated quite carefully in order to recapture that power.  (Also see Ibanez-Mejia et al. 2017 for a similar point).  Losing all the small-scale power is likely to substantially influence conclusions about coherent cores and the speed of collapse at early times.  At the very least, this point needs to be explicitly acknowledged in the discussion and conclusion.  Testing of this dramatic approximation would be better.

3.)
* Second, the lack of sink particles means that gas collapses to the grid scale and then remains at that density, effectively introducing a grid pressure. This behavior can clearly be seen in, for example, Figure 2, particularly panels 2 and 5.  This limitation is indeed explicitly acknowledged in the paper, but then it is not acted upon, as analysis is performed on cores well beyond the limit, with, for example, discussion of core interactions ("mosh"), rotating disks producing large tangential viscosities, and relaxed objects after singularity (Sect 4, 2nd para).  None of that behavior is resolved. The interacting cores would be far more compact objects less sensitive to tidal forces if collapse were allowed to continue. The apparent disks would be subject to strong magnetic braking if the field tensions could be resolved at those small scales (I also very much wonder if the disks ended up aligned with coordinate axes, as is typical of underresolved rotating flows). The only reason that a post-singularity object appears relaxed is because of support from grid pressure preventing it from collapsing to form one or more protostars.   My preferred solution to these issues would be to remove discussion of unresolved results from the paper, which would admittedly shorten it fairly dramatically; alternatively, the importance of the lack of resolution needs to be emphasized in terms of limits and bounds on behavior wherever unresolved results are described or discussed.

4.)
* Third, tracer particles in Godunov methods were shown by Genel et al. (2013) to be subject to unphysical clumping that can be relieved by using a Monte Carlo method to enforce statistically correct fluxes of particles across zone boundaries.  As there is no discussion of this issue here, I assume it is an issue that should be checked for its influence on the results.  If this isn't true, that should be explicitly demonstrated.

There were a couple of issues with the analysis that I'd also like to see addressed:

5.)
* In discussion of Table 1 in the second paragraph of Sect. 3.1, a trend of single cores being increasing common with increased magnetization is described.  However, examination of Table 1 reveals no such trend, with the intermediate magnetization case having far fewer single cores than either the low or high magnetization cases.

6.) 
* In sect 3.2, the claim is made, "By various theorems one learns in calculus, before the density gets large, the time derivative of density must becomes [sic] large."  Although I invite a more specific statement of the theorems being referenced, I strongly suspect that they do not exist.  Consider partial rho / partial t = 1 for a time of 10^5 time units.  This will reach a density of 10^5 just as well as any more dramatic increase in density over a shorter timescale. (The empirical statement made should have a citation; perhaps to Paper I?) Rather, this section just seems to be describing the consequences of gravitational collapse as described by Larson (1969), Penston (1969), Shu (1977), and finally in all generality, encompassing all the prior solutions, by Whitworth & Summers (1984).  I suggest reference to these works in describing the expected behavior of collapsing cores.

7.)
* The observed value of Delta t_sing = 0.1 t_ff might be directly derivable from the density scale chosen for the box of 1000 cm^-3, which presumably determines the value of t_ff and the density set by the grid pressure for the end of the singularity of 10^5 cm^-3.  The factor of 100 difference in density leads to a factor of 10 difference in the free-fall time, as it is proportional to the inverse square root of density.

8.)
* The r^-2 behavior of \bar{\rho} described below equation (6) is only coincidentally equivalent to the r^-2 profile of \rho(r).  To see what I mean, consider what the behavior of \bar{\rho} would be for an r^-3 profile of \rho(r). It would not produce a \bar{\rho} behavior of r^-3, as can be seen from direct integration of Eq 6!  In the same paragraph, I somehow doubt that singular isothermal spheres can be numerically resolved.  All that can actually be said is that the central flat regions have become small enough to no longer be resolvable with the limited available numerical resolution.

9.)
* Below equation (9) there is a claim that there should be a square-root dependence of the turbulent velocity on the radius. A citation should be provided for this claim.

10.)
* The discussion of virialization throughout the paper needs to be thought through a bit more:
1. A core supported by a combination of rotation and grid pressure is described as a "virialized object" in the abstract and conclusions, and elsewhere in the paper.  This is a pretty dramatic extension of the concept of virial equilibrium, one that I suggest is unwarranted and should not be included in the paper.  (See Ballesteros-Paredes et al. 2011b for a discussion of the difference between virial and free-fall dynamics).  
2. At the beginning of the paragraph following equation (4) on page 6, the value 2 is described as "the often quoted value for virialization."  It isn't explained *why* this is often quoted until the top of page 7.  That explanation should probably be provided immediately on citing the value of 2.

11.)
* An object is described (p. 8, line 57, first col) as "not a fractal mess (well less of a mess)".  Doesn't this actually mean that the fractal dimension is increasing towards 3?  Can this be demonstrated quantitatively in order to replace this highly qualitative description?

12.)
* In the conclusions, comparison is made to Offner et al. (2022).  However, they found that there was no well-determined time dependence of their three phases, with cores moving almost randomly between the different phases over time.  This seems perhaps distinct from the behavior described here.  If it isn't, that would be well worth emphasizing.

13.) 
* more discussion of how the cores modeled here compare to observed objects in scale and properties would be useful.

There are quite a number of issues with the presentation that need to be addressed:

14.)
* Terms and variables need to be defined on first use:
- cruise-then-collapse
- fractal dimension (quickly summarize the analysis method from Paper I as well)
- many-to-many
- $t_{\rm sung}$
- $t_{\rm ff}$ (make clear that this is the global value)
- plasma beta (should be defined in the text rather than the table)
- rho 

15.)
* subscripts functioning as labels should be set in roman, while subscripts that are variables can remain in italic. ($E_{\rm K}$ but $v_r$, for example)

16.)
*inline use of \sqrt is generally a bad idea.  Use ( ... )^{1/2}.

17.)
* watch out for the spaces before the units (eg in the first line of the text)

18.)
* instead of trying to include "few" in an equation on the second line of the text, write out the statement: velocity dispersion $\sigma_v$ of a few times the sound speed $c_{\rm s}$."

19.)
* page 1, line 42, col 2: the PDF suppression factor is not rho^{1/2}, which increases with density, but rather (rho/rho_max)^1/2, which decreases with density.

20.)
* Sect 2.2: Please offer some justification for the scaling chosen.  In particluar, molecular clouds near the Sun have average densities of 100 cm^-3, so the chosen value implies an extraordinarily dense cloud.  It would further be useful to explicitly give the full set of physical scaling factors for the chosen scaling, including the minimum and maximum cell sizes, the sound speed (velocity scale), and the free-fall time (also note that the variable $t_{\rm ff}$ is the global, not the local free-fall time.   

21.)
* In the referee's version, axis labels are cut off or overlapping with data in Figures 1 and 4.

22.)
* It might help the reader to add a panel to Figure 1 showing a different view of core 74 to emphasize its initially low fractal dimension nature.

23.)
* Every figure axis label needs units or scaling.
- Figure 1: if these are fractions of the full box size, define L to be that size and use x/L as your axis label.  Also specify somewhere where your zero point lies, to explain the negative x-value in the bottom left panel.
- Figure 2: Consider whether the variable rho should really have units of cm^-3, or whether it would be less confusing to use n for this variable.  Note that the same variable is called rho_{\rm particle} in Figure 9; I suggest unifying the notation (probably by dropping the subscript).
- Figure 3: are the horizontal axes in units of t_ff?  The vertical axes are clearly not N, but rather N/N_total, right?  I suggest not using the axis label to identify the simulation, but rather a label in the data area (if you move the legend to the bottom right of the figure, there will be space for simulation labels at the top left corners of the left hand column of panels.)
- Figure 4: all vertical axis units need to be given correctly.  Again, don't use axis labels to identify the plot, only to identify the values on the axis.
- Figures 5 & 7: can you get the subscripts working for the time scaling?
- Figure 6: units need to be given for all vertical axes (in the caption if the labels are too small).  The horizontal axis is scaled by a non-existent variable, presumably equivalent to t_{\rm sing}.
- Figure 8: units are given here.  However, for density, they are almost certainly wrong, as 10^8 g cm$^{-3}$ (preferred style rather than g/cc) is comparable to the interior of a white dwarf.  Likely the average number density \bar{n} in cm$^{-3}$ was meant, in which case that variable needs to be defined and used in place of \bar{\rho}.
- Figure 9: again, give distance unit.  Consider whether the variable rho_{\rm particle} should really have units of cm^-3, or whether it would be less confusing to define n_{\rm particle}.

24.)
* Section 3 intro: The adjective "alone" cannot be used before nouns in English, so an "alone core" is ungrammatical.  Please rename this class everywhere (eg to single or lone), or else rephrase to avoid the ungrammatical usage of alone everywhere that "alone core" is used.

25.)
* Section 3.1: what is the unit for \delta?  Why is this value chosen?

26.)
* Figure 4: define the three velocity types in the caption rather than in the text.

27.)
* rewrite section 3.3 to describe the table before drawing conclusions from it.  Note that a new definition of t_{\rm ff} for individual cores is introduced here, which is quite confusing.  Clarify that this is a different variable from the scaling factor used, for example, in Figure 2 (and many other places).

28.)
* Figure 5: color bar labels overlap at ends.  

29.)
* Section 3.4.3: The explanation given in Sect. 3.5.2 for the choice of 1000 AU as a fiducial radius should be moved forward to the first use of M_{1000} in Sect. 3.4.3

30.)
* Figure 7, caption uses the term "within 0.1t_ff of t_sing. How can this be seen from the plot, which is in fractions of t_sing, with no reference to t_ff?  Also, in the same caption, "All" should be revised to "Most", following the text description of the plot.


31.)
Finally, I just list the typos and grammatical or stylistic problems that need correcting:

page 1, line 32, column 1: comma after "10K)"

p1 l45 c2: primage

p2 l27 c1: adaptive mesh refinement isn't a capitalized proper noun

p2 l31 c1: why is L_J defined with rho_0 rather than the local density rho?  

p2 l51 c1: Mach is a capitalized proper noun

p3 l30 c1 Sections 3.4

p3 l48 c1 insert or before if.

p3 l32 c2 forth

p3 l44 c2 must becomes large

p5 l47 c1 4 -> Four

p8 l24 c1 make -> take

p11 l3 c1 present here

p11 l10 c1 NSF Astronomy grants have the prefix AST not AAG.


==> REPORT2.tex <==
Comments to the Author
The authors have made extensive revisions in response to my initial report.  There continue to be a few issues that need to be reconsidered prior to my recommending publication.  However, these issues are straightforward enough that I think they can be handled in a final revision that will not require my further review.

1.) 
The biggest issue is that the concept of virialization continues to be poorly described in the text.  The key point is that the virial equation describes energy conservation.  Thus, all forms of energy important in the system must be taken into account.  Equation (21) is thus only appropriate for a collisionless, pressure-free, unmagnetized system such as a gas-free star cluster.  The system considered here is nothing like that.  Instead, it has a far more complex complete virial equation, given in full by McKee & Zweibel (1992).  Simple approximations can be made.  If kinetic energy balances gravity in a hypersonic flow, and there are no significant surface terms, then equation (21) is maybe not terrible.  However, when thermal energy dominates, the virial equation reduces to a hydrostatic balance between thermal energy (pressure) and gravity, with kinetic energy unimportant.  This is the first hydrostatic core regime.  Thus, describing that core as virialized with reference to equation (21) is incomplete or even incorrect.  Rewriting the paragraph around equation (21) should handle this issue.

2.)
The next paragraph tries to draw an analogy with the stellar dynamical concept of violent relaxation.  Again, this is a concept that is only is relevant to pressure-free systems.  Bonilla-Barroso et al (2022) indeed consider violent relaxation in a star formation context, but they were considering the behavior of already formed stellar clusters within their clouds, not the behavior of self-gravitating gas. I suggest removal of this analogy (and the corresponding sentence in the conclusions).  As I did not flag this issue in my first report, I don't require this removal, but leaving it in may expose the authors to appropriate criticism.  If they want to make a much more detailed argument for the analogy that clearly shows that pressure is irrelevant in the system under study, that would be one alternative, though I don't expect that to be possible.

Aside from these two issues, there remain a number of minor issues of composition and grammar.  (Missing words or letters provided with [], suggested deletions using X...X)

Most widespread are violations of English sentence structure with both sentence fragments and run-on sentences appearing.

3.) 
run-on sentences:

Sect 2.2.2  ... sound speed, we assume...
Sect 3.1.1  ... are not the same, this is a tight...
Sect 3.1.1  ... threshold for collapse, by the time...
Sect 3.3.1  ... large converging flow, in fact some cores...
Figure 5 capt ... preferred initial configuration, some [cores] begin with...
Sect 4      ... is our selection bias, we only examine cores... 
           ... featureless distribution, the most that... 

4.)
sentence fragments:

Figure 5 capt ... Universally supersonic at...
Sect 4        ... One in which velocity of the gas that will collapse

Other issues:

5.)
In abstract: reference to final hydrostatic or rotationally supported object as virialized is misleading (as noted above)

6.)
Section 1
the standard notation for 1e-6 G is microgauss, not micro Gauss.

7.)
As I understand, coherent cores are not sub-virial, but subsonic.

8.)
The concept of a direct relationship between the core IMF and the stellar IMF has been strongly criticized on time-scale grounds by Clark, Klessen & Bonnell (2007), which needs to be mentioned if you want to introduce the concept.  (Also see Smith, Clark, & Bonnell 2009). 

9.)
filst -> first

10.)
showed that [a] sphere will collapse

11.)
There is a vast literature discussing the values of \alpha_v and \alpha_n, or even if these relations are anything but a special case of the Heyer relation. The 1981 values are certainly out of date. At some point, that literature needs to be absorbed into this project, whether in this paper or in the future.  Ballesteros-Paredes & Mac Low 2002 and Ballesteros-Paredes et al. 2011a are a fine place to start. 

12.)
third para from end \citep{collins23} -> \citet

Sect 2.1 & Sect 2.2.1

13.)
AMR, CT, and MHD are little-used or unused acronyms that should be removed from the paper.  (MHD isn't defined either.)

Sect. 2.2.2

14.)
that our XourX simulations

15.)
define the variable c explicilty

16.)
correct spacing of unit in equation 7 (should be $...0.2\mbox{ km s}...)

Sect. 2.3

17.)
correct unit spacing: 20AU

18.)
ILES is a little-used acronym and can be removed by rewriting. (e.g. "In such a simulation...")

Sect 2.4

19.)
sticking together the[y] efffectively

Sect 3.1.1

20.)
avoid use of stacked fractions in text.  Use a display equation if stacking is needed.

21.)
The first such stacked equation needs units for the numerical constant of 10^5.  (I'm rather concerned that the units are cm^-1 t_ff^-1, which is a rather horrifying mixed unit.)

22.)
in the same sentence, max -> maximum

23.)
two densities [is] proportional

Sect 3.1.2

24.)
The discussion in the text does not agree with the values in the table.  The correlation with local t_ff is just as good as the number of particles in the core. The number of particles does not reach R = -0.5.  Rather, only rho-bar in sim3 reaches this value.  The local free-fall time has a range 0.37 < R < 0.48, contradicting the assertion in the text that it has R < 0.2 in two simulations and 0.37 in the third.

Sect 3.2.1

25.)
the envelope [has a density profile proportional to] Xis aX $r^{-2}$

26.)
at the inner radius XandX [to]

Sect 3.2.2

27.)
gravitationalXlyX

Sect 3.3

28.)
clusterXsX cores

Sect 3.3.1

29.)
mean quantities [in] XonX preimage gas

30.)
choose a consistent abbreviation for root-mean-square (both r.m.s. and RMS are used in various places).

31.)
The text uses |\bar{v_{\rm radial}}| but the caption of Figure 5 neglects to include the absolute value signs.  Same for v_{\rm T}.

Figure 5 caption

32.)
increaseXdX

33.)
pr[e]image (twice, and again once elsewhere in text)

34.)
Radial velocity has noXtX preferred...

Sect 3.3.3

35.)
One set of brackets should be square in equations 22 & 23

Sect 3.3.5

36.)
psuedo -> pseudo

37.)
roughy -> roughly

39.)
The discussion of Figure 9 needs to explicitly describe the red lines in the text to fulfill the promise made at the end of the caption.  This is not currently done anywhere.

40.)
The scare quotes below equation 27 should be removed.  If doubt or deprecation is required, it should be provided by rewriting the text.

41.)
XisX becomes quite large...

Section 4

42.)
logarithmica[l]ly

43.)
(same sentence) providing a central value for E_K/E_G is quoting an unresolved value.

44.)
cores move between [all] phases  (This is a key point of Offner et al IMHO!)

45.)
Pelkonen et al. should be a \citep, not \citet

references:

46.)
the books cited need publication data


==> REPORT_eat.tex <==

Scientific Editor: Prof Andrew King





There were a couple of issues with the analysis that I'd also like to see addressed:

5.)
* In discussion of Table 1 in the second paragraph of Sect. 3.1, a trend of
single cores being increasing common with increased magnetization is described.
However, examination of Table 1 reveals no such trend, with the intermediate
magnetization case having far fewer single cores than either the low or high
magnetization cases.

6.)
* In sect 3.2, the claim is made, "By various theorems one learns in calculus,
before the density gets large, the time derivative of density must becomes [sic]
large."  Although I invite a more specific statement of the theorems being
referenced, I strongly suspect that they do not exist.  Consider partial rho /
partial t = 1 for a time of 10^5 time units.  This will reach a density of 10^5
just as well as any more dramatic increase in density over a shorter timescale.
(The empirical statement made should have a citation; perhaps to Paper I?)
Rather, this section just seems to be describing the consequences of
gravitational collapse as described by Larson (1969), Penston (1969), Shu
(1977), and finally in all generality, encompassing all the prior solutions, by
Whitworth & Summers (1984).  I suggest reference to these works in describing
the expected behavior of collapsing cores.


8.)
* The r^-2 behavior of \bar{\rho} described below equation (6) is only coincidentally equivalent to the r^-2 profile of \rho(r).  To see what I mean, consider what the behavior of \bar{\rho} would be for an r^-3 profile of \rho(r). It would not produce a \bar{\rho} behavior of r^-3, as can be seen from direct integration of Eq 6!  In the same paragraph, I somehow doubt that singular isothermal spheres can be numerically resolved.  All that can actually be said is that the central flat regions have become small enough to no longer be resolvable with the limited available numerical resolution.





=========== COME BACK TO THESE


10.)
* The discussion of virialization throughout the paper needs to be thought
through a bit more: 1. A core supported by a combination of rotation and grid
pressure is described as a "virialized object" in the abstract and conclusions,
and elsewhere in the paper.  This is a pretty dramatic extension of the concept
of virial equilibrium, one that I suggest is unwarranted and should not be
included in the paper.  (See Ballesteros-Paredes et al. 2011b for a discussion
of the difference between virial and free-fall dynamics).  2. At the beginning
of the paragraph following equation (4) on page 6, the value 2 is described as
"the often quoted value for virialization."  It isn't explained *why* this is
often quoted until the top of page 7.  That explanation should probably be
provided immediately on citing the value of 2.

12.)
* In the conclusions, comparison is made to Offner et al. (2022).  However, they
found that there was no well-determined time dependence of their three phases,
with cores moving almost randomly between the different phases over time.  This
seems perhaps distinct from the behavior described here.  If it isn't, that
would be well worth emphasizing.

22.)
* It might help the reader to add a panel to Figure 1 showing a different view
of core 74 to emphasize its initially low fractal dimension nature.
d.) Progress in p19_plots/fig_fractal.  Making slices with dots.  
d.) Also try p19_plots/fractals, which makes the covering boxes.








==> REPORT_response1.tex <==

Dear Mordecai--

Thanks for your careful read of our paper.  I value your opinion highly, and have tried to make all the improvements you suggest.  

I view this work as a pilot study.  Higher resolution simulations are in the pipe, but aren't far along enough to supplement the current publication.   This was a probe of what I could see with tracer particles, at a scale I could manage for this new technique.

I've done a substantial amount of editing of results, and it's a much better paper.  Some of what looked like bad analysis was actually bad exposition.  I've reworked how I discuss the numerical actuality of the collapse, to separate the grid-pressure supported mass, which is not at all resolved, from the envelope.  I've also taken care to stop analysis after the collapse.  

Please let me know what you think.  I think that with your help this is a much improved paper.  There is possibly still more room for improvement, I appreciate your input on this version.

I'll address your points in turn.

1.) Please ensure that all textual labels in figures are at least as large as the caption text; any smaller and they become too difficult to read.  

d.) I have done this as far as I can tell, please let me know if any need further adjustment.

2.) First, at the beginning of the run, a rather well-resolved model with 1024^3 zones is downsampled by an order of magnitude in linear resolution to 128^3 prior to turning on self-gravity.  The result of this downsampling, as emphasized by Seifried, Walch et al. (2017), is to erase the high-wavenumber end of the turbulent power spectrum.  The subsequent collapse and refinement has to be treated quite carefully in order to recapture that power.  (Also see Ibanez-Mejia et al. 2017 for a similar point).  Losing all the small-scale power is likely to substantially influence conclusions about coherent cores and the speed of collapse at early times.  At the very least, this point needs to be explicitly acknowledged in the discussion and conclusion.  Testing of this dramatic approximation would be better. 

d.) I completely agree, this is not a well resolved run.   I view this work as a pilot study.  I completely agree with your assessment of the reduction of small scale power.   I've added a bit in the conclusions section outlining how the results would be affected by better root grid resolution.   High resolution simulations are running right now and I'm training the grad student that will add the improved subgrid models, but those will take some time.

3.) * Second, the lack of sink particles means that gas collapses to the grid scale and then remains at that density, effectively introducing a grid pressure. This behavior can clearly be seen in, for example, Figure 2, particularly panels 2 and 5.  This limitation is indeed explicitly acknowledged in the paper, but then it is not acted upon, as analysis is performed on cores well beyond the limit, with, for example, discussion of core interactions ("mosh"), rotating disks producing large tangential viscosities, and relaxed objects after singularity (Sect 4, 2nd para).  None of that behavior is resolved. The interacting cores would be far more compact objects less sensitive to tidal forces if collapse were allowed to continue. The apparent disks would be subject to strong magnetic braking if the field tensions could be resolved at those small scales (I also very much wonder if the disks ended up aligned with coordinate axes, as is typical of underresolved rotating flows). The only reason that a post-singularity object appears relaxed is because of support from grid pressure preventing it from collapsing to form one or more protostars.   My preferred solution to these issues would be to remove discussion of unresolved results from the paper, which would admittedly shorten it fairly dramatically; alternatively, the importance of the lack of resolution needs to be emphasized in terms of limits and bounds on behavior wherever unresolved results are described or discussed.

d.) Hopefully I've cut out any objectionable analysis.  
I've also tried to be more explicit about what object I'm referring too, I wasn't always clear.

4.)
* Third, tracer particles in Godunov methods were shown by Genel et al. (2013) to be subject to unphysical clumping that can be relieved by using a Monte Carlo method to enforce statistically correct fluxes of particles across zone boundaries.  As there is no discussion of this issue here, I assume it is an issue that should be checked for its influence on the results.  If this isn't true, that should be explicitly demonstrated.

d.) This is definitely a process that we see, but not one that's a problem for us in this work.  We've added a bit of text to explain.  In brief, particles clump because, when in a region of converging flow, are driven to zero separation quickly.   Once closer than one zone, two particles are not likely to be separated by the spatially linear (not turbulent) velocity field. For us this is a feature, not a bug, since we're selecting gas that is in highly convergent flow for its entire lifetime; they can stick all they like.  Since the particles "stick" together, they don't inject any more small scale noise that would ruin the causal relation of the gas along the particle path.  Post collapse, no analysis is done that requires the particles' information other than the one zone they all occupy.  It's effectively like removing them from the simulation by way of accreting onto a subgrid model.  

There were a couple of issues with the analysis that I'd also like to see addressed:

5.)
* In discussion of Table 1 in the second paragraph of Sect. 3.1, a trend of single cores being increasing common with increased magnetization is described.  However, examination of Table 1 reveals no such trend, with the intermediate magnetization case having far fewer single cores than either the low or high magnetization cases. 

d.) The truth of that statement changed as the mode technique evolved.  I've removed it.

6.) 
* In sect 3.2, the claim is made, "By various theorems one learns in calculus, before the density gets large, the time derivative of density must becomes [sic] large."  Although I invite a more specific statement of the theorems being referenced, I strongly suspect that they do not exist.  Consider partial rho / partial t = 1 for a time of 10^5 time units.  This will reach a density of 10^5 just as well as any more dramatic increase in density over a shorter timescale. (The empirical statement made should have a citation; perhaps to Paper I?) Rather, this section just seems to be describing the consequences of gravitational collapse as described by Larson (1969), Penston (1969), Shu (1977), and finally in all generality, encompassing all the prior solutions, by Whitworth & Summers (1984).  I suggest reference to these works in describing the expected behavior of collapsing cores. 
d.) We've improved all of these things.  The exposition at the beginning is now improved, and I've made some more explicit connection to free fall collapse.   I have a goal of making a more explicit connection to the WS85 collapse solutions, but I'm not going to be able to make that happen in time for this paper. (and, frankly, that should be done on more well resolved simulations)

7.)
* The observed value of Delta t_sing = 0.1 t_ff might be directly derivable from the density scale chosen for the box of 1000 cm^-3, which presumably determines the value of t_ff and the density set by the grid pressure for the end of the singularity of 10^5 cm^-3.  The factor of 100 difference in density leads to a factor of 10 difference in the free-fall time, as it is proportional to the inverse square root of density.
d.) This is a great idea.   I've included such a discussion in the appropriate section.  

8.)
* The r^-2 behavior of \bar{\rho} described below equation (6) is only coincidentally equivalent to the r^-2 profile of \rho(r).  To see what I mean, consider what the behavior of \bar{\rho} would be for an r^-3 profile of \rho(r). It would not produce a \bar{\rho} behavior of r^-3, as can be seen from direct integration of Eq 6!  In the same paragraph, I somehow doubt that singular isothermal spheres can be numerically resolved.  All that can actually be said is that the central flat regions have become small enough to no longer be resolvable with the limited available numerical resolution. 
d.) I think it's more than coincidence; r^{-3} \int r^{a} r^{2} dr = r^{a} for a!= 3.  However, I don't actually need this to be the interior average, so we've replaced it with the azimuthal average.  This is one instance of my bad description, the bit at the center I agree is not trust worthy.  I didn't intend to say that the thing in the center is SIS, it's only 3 zones across.  The remaining envelope is several dissipation lengths across, so while more resolution would be better, it's not peanut butter.


9.)
* Below equation (9) there is a claim that there should be a square-root dependence of the turbulent velocity on the radius. A citation should be provided for this claim.
d.) We have added 2 references and fixed this up so its more clear.  

10a.)
* The discussion of virialization throughout the paper needs to be thought through a bit more: 
1. A core supported by a combination of rotation and grid pressure is described as a "virialized object" in the abstract and conclusions, and elsewhere in the paper.  This is a pretty dramatic extension of the concept of virial equilibrium, one that I suggest is unwarranted and should not be included in the paper.  (See Ballesteros-Paredes et al. 2011b for a discussion of the difference between virial and free-fall dynamics).  
d.) I agree with what you say.  This is mostly bad prose on my part, I didn't intend to say that the junk at the center is virialized, but the envelope which is resolved by several dissipation lengths is.  The extent to which 2K+U=0=1/2\ddot{I} is the extent to which the configuration of the envelope is evolving, so I feel ok refering to the envelope as a relaxed object. I've removed most of the references to virialization.

10b.)
2. At the beginning of the paragraph following equation (4) on page 6, the value 2 is described as "the often quoted value for virialization."  It isn't explained *why* this is often quoted until the top of page 7.  That explanation should probably be provided immediately on citing the value of 2.
d.) This got cleaned up with the previous point.

11.)
* An object is described (p. 8, line 57, first col) as "not a fractal mess (well
less of a mess)".  Doesn't this actually mean that the fractal dimension is
increasing towards 3?  Can this be demonstrated quantitatively in order to
replace this highly qualitative description?
d.)  I've removed this sentence, in favor of a section discussing
fractal dimension vs. time in a quantitative sense.  


12.) 
* In the conclusions, comparison is made to Offner et al. (2022).  However, they found that there was no well-determined time dependence of their three phases, with cores moving almost randomly between the different phases over time.  This seems perhaps distinct from the behavior described here.  If it isn't, that would be well worth emphasizing.
d.) I've added a possible interpretation.  

13.)
* more discussion of how the cores modeled here compare to observed objects in scale and properties would be useful.
d.) I've improved this.  There's now a more explicit interpretation of units,
and a better discussion of what is analyzed.


14.)
* Terms and variables need to be defined on first use:
- cruise-then-collapse
- fractal dimension (quickly summarize the analysis method from Paper I as well)
- many-to-many
- $t_{\rm sung}$
- $t_{\rm ff}$ (make clear that this is the global value)
- plasma beta (should be defined in the text rather than the table)
- rho 
d.) Hopefuly I've made everythig clear.  For the fractal dimension reference in
the introduction, I include more prose in the body and add a reference.  


15.)
* subscripts functioning as labels should be set in roman, while subscripts that
are variables can remain in italic. ($E_{\rm K}$ but $v_r$, for example)
d.) Thanks, I've corrected this.

16.)
*inline use of \sqrt is generally a bad idea.  Use ( ... )^{1/2}.
d.) This improvement has been made.

17.)
* watch out for the spaces before the units (eg in the first line of the text)
d.) I've done my best.

18.)
* instead of trying to include "few" in an equation on the second line of the
text, write out the statement: velocity dispersion $\sigma_v$ of a few times the
sound speed $c_{\rm s}$."
d.) This has been rewritten.

19.)
* page 1, line 42, col 2: the PDF suppression factor is not rho^{1/2}, which
increases with density, but rather (rho/rho_max)^1/2, which decreases with
density.
d.) A good point, this has been fixed.

20.)
* Sect 2.2: Please offer some justification for the scaling chosen.  In
particluar, molecular clouds near the Sun have average densities of 100 cm^-3,
so the chosen value implies an extraordinarily dense cloud.  It would further be
useful to explicitly give the full set of physical scaling factors for the
chosen scaling, including the minimum and maximum cell sizes, the sound speed
(velocity scale), and the free-fall time (also note that the variable $t_{\rm
ff}$ is the global, not the local free-fall time.   
d.) This density was chosen to make the Mach number consistent with Larson's
laws.    I do agree this is a relatively dense, but that's because
it's a  relatively high Mach number.  
I had stuck with these units to be
consistent with the 2012 paper.  Now that I look back, though, I am not sure how
Alexi and I arrived at a length of 4.6 pc.  Now I get a length of 3.6 pc and a density of
817.  
I've replotted with these lower values, and added a more complete justification
in the paper.

21.)
* In the referee's version, axis labels are cut off or overlapping with data in Figures 1 and 4.
d.) These have been fixed.

22.)
* It might help the reader to add a panel to Figure 1 showing a different view of core 74 to emphasize its initially low fractal dimension nature.
d.) I decided to remove this figure.

23.)
* Every figure axis label needs units or scaling.
x - Figure 1: if these are fractions of the full box size, define L to be that size and use x/L as your axis label.  Also specify somewhere where your zero point lies, to explain the negative x-value in the bottom left panel.
x - Figure 2: Consider whether the variable rho should really have units of cm^-3, or whether it would be less confusing to use n for this variable.  Note that the same variable is called rho_{\rm particle} in Figure 9; I suggest unifying the notation (probably by dropping the subscript).
x - Figure 3: are the horizontal axes in units of t_ff?  The vertical axes are clearly not N, but rather N/N_total, right?  I suggest not using the axis label to identify the simulation, but rather a label in the data area (if you move the legend to the bottom right of the figure, there will be space for simulation labels at the top left corners of the left hand column of panels.)
X - Figure 4: all vertical axis units need to be given correctly.  Again, don't use axis labels to identify the plot, only to identify the values on the axis.
X - Figures 5 & 7: can you get the subscripts working for the time scaling?
X - Figure 6: units need to be given for all vertical axes (in the caption if the labels are too small).  The horizontal axis is scaled by a non-existent variable, presumably equivalent to t_{\rm sing}.
X - Figure 8: units are given here.  However, for density, they are almost certainly wrong, as 10^8 g cm$^{-3}$ (preferred style rather than g/cc) is comparable to the interior of a white dwarf.  Likely the average number density \bar{n} in cm$^{-3}$ was meant, in which case that variable needs to be defined and used in place of \bar{\rho}.
X - Figure 9: again, give distance unit.  Consider whether the variable rho_{\rm particle} should really have units of cm^-3, or whether it would be less confusing to define n_{\rm particle}.
d.) We have addressed these issues.




24.)
* Section 3 intro: The adjective "alone" cannot be used before nouns in English, so an "alone core" is ungrammatical.  Please rename this class everywhere (eg to single or lone), or else rephrase to avoid the ungrammatical usage of alone everywhere that "alone core" is used.
d.) An excellent point.  I've replaced "alone" with "single" throughout.

25.)
* Section 3.1: what is the unit for \delta?  Why is this value chosen?
d.) We have added some more details about $\delta$ in Section 3.1.

26.)
* Figure 4: define the three velocity types in the caption rather than in the text.
d.) Done.

27.)
* rewrite section 3.3 to describe the table before drawing conclusions from it.
Note that a new definition of t_{\rm ff} for individual cores is introduced
here, which is quite confusing.  Clarify that this is a different variable from
the scaling factor used, for example, in Figure 2 (and many other places).
d.) We have made these improvements.

28.)
* Figure 5: color bar labels overlap at ends.  
d.) We have improved the color bar.

29.)
* Section 3.4.3: The explanation given in Sect. 3.5.2 for the choice of 1000 AU
as a fiducial radius should be moved forward to the first use of M_{1000} in
Sect. 3.4.3
d.) Yes, we have fixed this.  

30.)
* Figure 7, caption uses the term "within 0.1t_ff of t_sing. How can this be
seen from the plot, which is in fractions of t_sing, with no reference to t_ff?
Also, in the same caption, "All" should be revised to "Most", following the text
description of the plot.
d.) That's a good point, you actually can't see it from this plot but you can
from Figure 3.  I've fixed "most" and added a reference to Figure 3.


31.)  Typos
d.) We have fixed all of the typos.
page 1, line 32, column 1: comma after "10K)"

X p1 l45 c2: primage

X p2 l27 c1: adaptive mesh refinement isn't a capitalized proper noun

X p2 l31 c1: why is L_J defined with rho_0 rather than the local density rho?  

X p2 l51 c1: Mach is a capitalized proper noun

X p3 l30 c1 Sections 3.4

X p3 l48 c1 insert or before if.

X p3 l32 c2 forth

X p3 l44 c2 must becomes large

X p5 l47 c1 4 -> Four

X  p8 l24 c1 make -> take

X p11 l3 c1 present here

X p11 l10 c1 NSF Astronomy grants have the prefix AST not AAG.


==> REPORT_response2.tex <==
Dear Mordecai--

Thanks again for your careful read of our paper.  I've addressed your remaining concerns. I've removed the bits about relaxation and fixed the remaining typesetting and wording issues.  I appreciate your time and care.


Comments to the Author
The authors have made extensive revisions in response to my initial report.  There continue to be a few issues that need to be reconsidered prior to my recommending publication.  However, these issues are straightforward enough that I think they can be handled in a final revision that will not require my further review.

1.) 
The biggest issue is that the concept of virialization continues to be poorly described in the text.  The key point is that the virial equation describes energy conservation.  Thus, all forms of energy important in the system must be taken into account.  Equation (21) is thus only appropriate for a collisionless, pressure-free, unmagnetized system such as a gas-free star cluster.  The system considered here is nothing like that.  Instead, it has a far more complex complete virial equation, given in full by McKee & Zweibel (1992).  Simple approximations can be made.  If kinetic energy balances gravity in a hypersonic flow, and there are no significant surface terms, then equation (21) is maybe not terrible.  However, when thermal energy dominates, the virial equation reduces to a hydrostatic balance between thermal energy (pressure) and gravity, with kinetic energy unimportant.  This is the first hydrostatic core regime.  Thus, describing that core as virialized with reference to equation (21) is incomplete or even incorrect.  Rewriting the paragraph around equation (21) should handle this issue.

d.) I've removed this paragraph, leaving it as "near equillibration of energies" rather than virialization.  I'll write a proper paper on this topic shortly and with better simulations.

2.)
The next paragraph tries to draw an analogy with the stellar dynamical concept of violent relaxation.  Again, this is a concept that is only is relevant to pressure-free systems.  Bonilla-Barroso et al (2022) indeed consider violent relaxation in a star formation context, but they were considering the behavior of already formed stellar clusters within their clouds, not the behavior of self-gravitating gas. I suggest removal of this analogy (and the corresponding sentence in the conclusions).  As I did not flag this issue in my first report, I don't require this removal, but leaving it in may expose the authors to appropriate criticism.  If they want to make a much more detailed argument for the analogy that clearly shows that pressure is irrelevant in the system under study, that would be one alternative, though I don't expect that to be possible.

d.) I've removed this section.  I'll write a better paper on this idea.

Aside from these two issues, there remain a number of minor issues of composition and grammar.  (Missing words or letters provided with [], suggested deletions using X...X)

Most widespread are violations of English sentence structure with both sentence fragments and run-on sentences appearing.

3.) 
run-on sentences:

Sect 2.2.2  ... sound speed, we assume...
Sect 3.1.1  ... are not the same, this is a tight...
Sect 3.1.1  ... threshold for collapse, by the time...
Sect 3.3.1  ... large converging flow, in fact some cores...
Figure 5 capt ... preferred initial configuration, some [cores] begin with...
Sect 4      ... is our selection bias, we only examine cores... 
           ... featureless distribution, the most that... 
d.) These have been fixed.

4.)
sentence fragments:

Figure 5 capt ... Universally supersonic at...
Sect 4        ... One in which velocity of the gas that will collapse
d.) Fixed

Other issues:

5.)
In abstract: reference to final hydrostatic or rotationally supported object as virialized is misleading (as noted above)
d.) Fixed.

6.)
Section 1
the standard notation for 1e-6 G is microgauss, not micro Gauss.
d.) Fixed.

7.)
As I understand, coherent cores are not sub-virial, but subsonic.
d.) Yes, I've fixed that.

8.)
The concept of a direct relationship between the core IMF and the stellar IMF has been strongly criticized on time-scale grounds by Clark, Klessen & Bonnell (2007), which needs to be mentioned if you want to introduce the concept.  (Also see Smith, Clark, & Bonnell 2009). 
d.) An excellent point, I've added a reference and softened that point.

9.)
filst -> first
d.)  fixed.

10.)
showed that [a] sphere will collapse
d.) fixed.

11.)
There is a vast literature discussing the values of \alpha_v and \alpha_n, or even if these relations are anything but a special case of the Heyer relation. The 1981 values are certainly out of date. At some point, that literature needs to be absorbed into this project, whether in this paper or in the future.  Ballesteros-Paredes & Mac Low 2002 and Ballesteros-Paredes et al. 2011a are a fine place to start. 
d.) I've improved that section with more modern work.  I'll leave the scaling to
physical units alone, as updating those numbers won't change the results in this
paper in a meaningful way.


12.)
third para from end \citep{collins23} -> \citet
d.) fixed

Sect 2.1 & Sect 2.2.1

13.)
AMR, CT, and MHD are little-used or unused acronyms that should be removed from the paper.  (MHD isn't defined either.)
d.) removed.

Sect. 2.2.2

14.)
that our XourX simulations
d.) fixed

15.)
define the variable c explicilty
d.) Fixed

16.)
correct spacing of unit in equation 7 (should be $...0.2\mbox{ km s}...$)
d.) Fixed all of those eqns.

Sect. 2.3

17.)
correct unit spacing: 20AU
d.) fixed.

18.)
ILES is a little-used acronym and can be removed by rewriting. (e.g. "In such a simulation...")
d.) fixed.

Sect 2.4

19.)
sticking together the[y] efffectively
d.) fixed

Sect 3.1.1

20.)
avoid use of stacked fractions in text.  Use a display equation if stacking is needed.
d.) fixed.

21.)
The first such stacked equation needs units for the numerical constant of 10^5.  (I'm rather concerned that the units are cm^-1 t_ff^-1, which is a rather horrifying mixed unit.)
d.) Yes, n0 doesn't make any sense.  I've fixed these units.  


22.)
in the same sentence, max -> maximum
d.) fixed.

23.)
two densities [is] proportional
d.) fixed.

Sect 3.1.2

24.)
The discussion in the text does not agree with the values in the table.  The correlation with local t_ff is just as good as the number of particles in the core. The number of particles does not reach R = -0.5.  Rather, only rho-bar in sim3 reaches this value.  The local free-fall time has a range 0.37 < R < 0.48, contradicting the assertion in the text that it has R < 0.2 in two simulations and 0.37 in the third.
d.) I've reworked that paragraph.  

Sect 3.2.1

25.)
the envelope [has a density profile proportional to] Xis aX $r^{-2}$
d.)

26.)
at the inner radius XandX [to]
d.) fixed

Sect 3.2.2

27.)
gravitationalXlyX
d.) fixed

Sect 3.3

28.)
clusterXsX cores
d.) fixed.  (decided that the problem was the word cores)

Sect 3.3.1

29.)
mean quantities [in] XonX preimage gas
d.)  Fixed.

30.)
choose a consistent abbreviation for root-mean-square (both r.m.s. and RMS are used in various places).
d.) chosen.

31.)
The text uses |\bar{v_{\rm radial}}| but the caption of Figure 5 neglects to include the absolute value signs.  Same for v_{\rm T}.
d.) fixed.

Figure 5 caption

32.)
increaseXdX
d.) fixed

33.)
pr[e]image (twice, and again once elsewhere in text)
d.) fixed

34.)
Radial velocity has noXtX preferred...
d.) fixed

Sect 3.3.3

35.)
One set of brackets should be square in equations 22 & 23
d.) Fixed

Sect 3.3.5

36.)
psuedo -> pseudo
d.) fixed

37.)
roughy -> roughly
d.) Fixed.

39.)
The discussion of Figure 9 needs to explicitly describe the red lines in the text to fulfill the promise made at the end of the caption.  This is not currently done anywhere.
d.) This has been fixed.

40.)
The scare quotes below equation 27 should be removed.  If doubt or deprecation is required, it should be provided by rewriting the text.
d.) It is better without the quotes, I did not intend to be casting doubt there.

41.)
XisX becomes quite large...
d.) fixed

Section 4

42.)
logarithmica[l]ly
d.) fixed.

43.)
(same sentence) providing a central value for E_K/E_G is quoting an unresolved value.
d.) Didn't really mean center, changed to "edge of pseudo-core."  

44.)
cores move between [all] phases  (This is a key point of Offner et al IMHO!)
d.) fixed

45.)
Pelkonen et al. should be a \citep, not \citet
d.) fixed

references:

46.)
the books cited need publication data
d.) fixed


==> fig_hair.tex <==
\begin{figure} \begin{center}
	\input{fig_hair_img}
\caption[ ]{The particle paths for several representative cores.  The top two panels show
core 214 and core 74, which are both single objects. Cores 112 and 113 are a binary on the bottom left panel, and can
be seen unmixing as collapse proceedes.  The bottom right panel shows a cluster of 5
cores, this time showing only the centroids of the cores, which can be seen
orbiting each other as they travel and collapse.  }
\label{fig.hair} \end{center} \end{figure}


==> fig_hair_img.tex <==
\includegraphics[width=\hw\textwidth]{figures/F1_hair.pdf}


==> fig_mosh.tex <==
\begin{figure} \begin{center}
	\includegraphics[width=\hw\textwidth]{figures/u502_mosh_x_c0009.png}
\caption[ ]{(\emph{Top}) Path lines for all particles for \emph{cluster} core 9 from \simb.
Particles begin at the dots and end on the red point at the bottom.  Multiple
centers of collapse can be seen, which aggregate until a close encounter ejects
the newly formed core from the cluster.  (\emph{Middle}) a close up of the late
stage tidal dynamics.  (\emph{Bottom}) As in Figure
\ref{fig.anatomy}, particle density (right axis) and velocity (left axis), with
(total, tangential, radial) velocity in (black, teal, red).  The tidal dynamics
before the ejection dominate the velocity signal.  Mean velocities go to zero
as the particles are all driven into a single zone.  }
\label{fig.mosh} \end{center} \end{figure}


==> methods_observations.tex <==
\subsection{Comparison with Observations}

These simulations are moderate resolution and highly idealized, but they're
still able to reproduce the main properties of observed cores.  This was
demonstrated in \citet{Collins11}, wherein we performed simulations with similar
resolution, refinement, mass, and Mach number.  In this work, we compared the
magnetic field and column density relation to the cores observed by
\citet{Falgarone08} and \citet{Troland08}, finding comparable values of $\sim 1
\mu$G and column densities of $\sim 10^{23} \rm{cm}^{-2}$.  We also compared the
mass distribution to the observed distribution by \citet{Enoch08}, finding a
comparable distribution of masses.


==> mnras_toc.tex <==

% The MNRAS class isn't designed to include a table of contents, but for this document one is useful.
% I therefore have to do some kludging to make it work without masses of blank space.
\begingroup
\let\clearpage\relax
\tableofcontents
\endgroup
\newpage


==> old/discussion.tex <==
\section{\red{Discussion}}

This work should be considered a numerical experiment, rather than a proper star
formation simulation, due to its low resolution and simplified physics.  Here we
will discuss the expectation how the results presented here will be impacted by
improved resolution and physics.

\begin{enumerate}
\item Initial resolution.  Loss of small scale power.
\item Lack of sinks or proper equation of state.  
\item Tracer clumping.
\end{enumerate}

The low root grid resolution will impact the major results in the following
ways.  The primary deficit is lack of small scale power in the velocity field
\begin{enumerate}
\item {\bf Preimage} As we showed in the first paper, the preimage region for a given star comes from several velocity
correlation lengths, which is much larger than the dissipation scale. Thus the
main selection of preimage gas will not be substantially affected by the lack of
small scale power.
\item {\bf Fractals and Mixing} From Paper I, the mixing between cores and the
fractal nature of the preimage gas will only be made more severe with enhanced
small-scale velocity.
\item {\bf Mode distribution} will likely be affected by enhanced small scale
power, as chaotic dynamics will alter the trajectories of individual collapsing
stars. Thus the detailed ratio of pseudo-stars in each mode is not a reliable
result, though the existence of three modes will not change.
\item {\bf  Collection, hardening and singularity} will be unaffected
qualitatively by small scale power; the bulk initial flow is determined by large
scale features that are unable to collapse initially due to mismatch between
kinetic and gravitational energies.  It will take some time for the mismatch to
resolve itself and the object to be ready to collapse, so the hardening phase is
still likely to persist in future studies.  The singularity itself is
inevitable.  Increasing small scale velocity power will not affect this behavior
qualitatively.  
\item {\bf Fast mass delivery} This will also not likely change with enhanced
root grid power, as the velocity is eventually dominated by converging flows that will be
larger in value than the turbulence.  The details of the peak density will be
altered by the inclusion of either sinks or a proper equation of state.
\item {\bf Collapse Rate}  The time scale for collapse is broadly distributed
through the duration of the simulation, and not strongly correlated with any
bulk properties of the preimage gas.  The timescale will possibly be delayed by
enhanced small scale velocity, but the bredth of the distribution will not
change.  Increased resolution will make the chaos more pronounced, it is highly
unlikely for a prefered timescale to emerge.
\item {\bf Fast relaxation of the surrounding core} This will also not likely be
affected by enhanced small scale power.
\end{enumerate}


==> old/mosh.tex <==








==> old/multiples.tex <==
\subsection{Multiples and Mosh}
\label{sec.multiples}

Until now, we have focused on cores that are \emph{single}.  When stretched to their
singularity time, a clear behavior of velocity decay followed by violent
relaxation is seen.  
Binaries and clusters exhibit
similar properties, with a few exceptions.  It should be noted that the ultimate
fate of binaries and clusters is not known to us, as we only simulate a short
duration in time.  

Binaries in our simulation are observed to form in one of two ways.  Either one
singularity forms, which then breaks into two as the large orbital kinetic energy it
gained by falling down the potential well breaks the object in two; or two
singularities form in the same basin, which then begin to orbit one another.  In both
cases, the behavior is similar to that described in Section \ref{sec.case_study}.  A future study will explore more details.  

Clusters similarly form multiple singularities, some of which fragment, and some
of which merge, and some of which cause substantial tidal torques on other
cores.  Many of these do not show the same transition to coherence that is seen
in lone or binary cores.    We examine one particularly large cluster core in
detail to demonstrate the differences that exist.

Figure \ref{fig.mosh}  shows the fourth phase, \emph{mosh}, using
core 9 from \simb.  This core is a member of a cluster with
several other cores, none of which are shown.  In these three figures, every particle is
plotted with a grey line that has an opacity of 0.1, meaning that as they
overlap
in space the lines get darker.  As particles collapse,
many particles are compressed into the same zone \citep{Collins23}, which makes the lines darker
proportional to the number of particles in the zone, and proportional to the
density in the zone.  In the top plot, we see
the entire collapse from $t=0$ (grey points) to the end (red point at
y=0.1 z=0.05).  The second panel shows a zoom-in of the pink region denoted in
the top panel. This shows sub clumps forming, orbiting each other, merging, and
getting ejected by a close encounter with other cores.  

The bottom panel of Figure \ref{fig.mosh} shows
density (right axis) and velocity (left axis) as in Figure \ref{fig.anatomy}.
The mean radial and tangential velocities are quite large until the core is
ejected from the cluster at $t=0.8 \tff$, after which the velocity dispersion is
zero due to the fact that all the particles occupy a single zone.  The r.m.s.
velocity is always extremely large because of the orbital dynamics of sub clumps,
which in this analysis framework are all treated as one.    It is possible that
the sub clumps do transition to coherence and we are unable to see it;  it is
possible that they don't, and there are multiple channels for star formation.  We will address this in a future work.



==> old_bibs/old.bib.0 <==
@ARTICLE{2002ApJ...570..734B,
       author = {{Ballesteros-Paredes}, Javier and {Mac Low}, Mordecai-Mark},
        title = "{Physical versus Observational Properties of Clouds in Turbulent Molecular Cloud Models}",
      journal = {\apj},
     keywords = {ISM: Clouds, ISM: Kinematics and Dynamics, Stars: Formation, Turbulence, Astrophysics},
         year = 2002,
        month = may,
       volume = {570},
       number = {2},
        pages = {734-748},
          doi = {10.1086/339624},
archivePrefix = {arXiv},
       eprint = {astro-ph/0108136},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...570..734B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> old_bibs/old.bib.1 <==
@ARTICLE{2011MNRAS.411...65B,
       author = {{Ballesteros-Paredes}, Javier and {Hartmann}, Lee W. and {V{\'a}zquez-Semadeni}, Enrique and {Heitsch}, Fabian and {Zamora-Avil{\'e}s}, Manuel A.},
        title = "{Gravity or turbulence? Velocity dispersion-size relation}",
      journal = {\mnras},
     keywords = {turbulence, stars: formation, ISM: clouds, ISM: general, ISM: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = feb,
       volume = {411},
       number = {1},
        pages = {65-70},
          doi = {10.1111/j.1365-2966.2010.17657.x},
archivePrefix = {arXiv},
       eprint = {1009.1583},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.411...65B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> old_bibs/old.bib.2 <==
@ARTICLE{2013MNRAS.436.3247K,
       author = {{Kritsuk}, Alexei G. and {Lee}, Christoph T. and {Norman}, Michael L.},
        title = "{A supersonic turbulence origin of Larson's laws}",
      journal = {\mnras},
     keywords = {turbulence, methods: numerical, stars: formation, ISM: structure, Astrophysics - Galaxy Astrophysics},
         year = 2013,
        month = dec,
       volume = {436},
       number = {4},
        pages = {3247-3261},
          doi = {10.1093/mnras/stt1805},
archivePrefix = {arXiv},
       eprint = {1309.5926},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.436.3247K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> old_bibs/old.bib.3 <==
@ARTICLE{2009ApJ...699.1092H,
       author = {{Heyer}, Mark and {Krawczyk}, Coleman and {Duval}, Julia and {Jackson}, James M.},
        title = "{Re-Examining Larson's Scaling Relationships in Galactic Molecular Clouds}",
      journal = {\apj},
     keywords = {ISM: clouds, ISM: kinematics and dynamics, Astrophysics},
         year = 2009,
        month = jul,
       volume = {699},
       number = {2},
        pages = {1092-1103},
          doi = {10.1088/0004-637X/699/2/1092},
archivePrefix = {arXiv},
       eprint = {0809.1397},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...699.1092H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> old_bibs/old.bib.4 <==
@ARTICLE{2007MNRAS.379...57C,
       author = {{Clark}, Paul C. and {Klessen}, Ralf S. and {Bonnell}, Ian A.},
        title = "{Clump lifetimes and the initial mass function}",
      journal = {\mnras},
     keywords = {stars: formation, stars: mass function, stars: pre-main-sequence, ISM: clouds, Astrophysics},
         year = 2007,
        month = jul,
       volume = {379},
       number = {1},
        pages = {57-62},
          doi = {10.1111/j.1365-2966.2007.11896.x},
archivePrefix = {arXiv},
       eprint = {0704.2837},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.379...57C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> old_bibs/old.bib.5 <==
@ARTICLE{2024ApJ...961..153C,
       author = {{Cahlon}, Shlomo and {Zucker}, Catherine and {Goodman}, Alyssa and {Lada}, Charles and {Alves}, Jo{\~a}o},
        title = "{A Parsec-scale Catalog of Molecular Clouds in the Solar Neighborhood Based on 3D Dust Mapping: Implications for the Mass-Size Relation}",
      journal = {\apj},
     keywords = {Molecular clouds, Solar neighborhood, Star forming regions, Scaling relations, 1072, 1509, 1565, 2031, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = feb,
       volume = {961},
       number = {2},
          eid = {153},
        pages = {153},
          doi = {10.3847/1538-4357/ad0cf8},
archivePrefix = {arXiv},
       eprint = {2308.14794},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...961..153C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> old_bibs/old.bib.7 <==
@ARTICLE{2019MNRAS.490.2648B,
       author = {{Ballesteros-Paredes}, J. and {Rom{\'a}n-Z{\'u}{\~n}iga}, C. and {Salom{\'e}}, Q. and {Zamora-Avil{\'e}s}, M. and {Jim{\'e}nez-Donaire}, M.~J.},
        title = "{What is the physics behind the Larson mass-size relation?}",
      journal = {\mnras},
     keywords = {turbulence, stars: formation, ISM: clouds, ISM: kinematics and dynamics, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {490},
       number = {2},
        pages = {2648-2655},
          doi = {10.1093/mnras/stz2575},
archivePrefix = {arXiv},
       eprint = {1909.03175},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.490.2648B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> vs_tsing.tex <==
\section{Things Not Correlated with \tsing}

The duration of the cruise phase, \tsing,  does not seem to be correlated with
any ``obvious'' quantity in the gas except for the number of particles in the
core, and that only weakly.  Here we 

We examine correlation between a quantity, $Q$ and the rate of collapse by way
of the Pearson $r$ between the mass weighted average of $Q$ for each core
and their respective singularity times.  Thus for each core, $c$, 
\begin{align}
\bar{Q_c} &= \sum_i Q_i \rho_i \Delta v_i/\sum_i \rho_i \Delta v_i\\
\end{align}
where the sum is taken over particles in core $c$.
The correlation is defined as
\begin{align}
r_{Q \tsing} = \frac{\sum_c (Q_c - \bar{Q_c})(\tsing-\bar{\tsing})}{\sqrt{
\sum_c \left(Q_c-\bar{Q_c}\right)^2 \sum_c \left(\tsing - \bar{\tsing}\right)
}}.
\end{align}
The value of $r_{Q \tsing}$ can range between $\pm 1$.  

We do this on the first frame.

We list the values of $r_{Q \tsing}$ in Table \ref{table2}.
$V_{\rm{particles}}$ is the volume subtended by the particles, which by
construction of our initial conditions is simply proportional to the number of
particles.  It is the most correlated.  The sign of the correlation indicates
that more particles gives a shorter collapse time.  As discussed in
\citet{Collins22}, the particles are distributed in a fractal manner in the
cloud.  $V_{\rm{hull}}$ is the volume of the convex hull bounding the
preimage particles. In brief, the convex hull is a polyhedron that bounds the
particles,  see \citet{Collins22} for a discussion.  This measures the extent of
the particles, ignoring the small volume filling fraction.  This is more weakly
correlated.   Average density, $\langle\rho\rangle$, specific gravitational
energy ($\EG/V$), and specific kinetic energy ($\EK/V$) are weakly negatively
correlated collapse time.  The total velocity, $v_{3d}$ is not correlated with
collapse time, nor is radial velocity $v_r$.  Tangential velocity, $v_t$, is also not
correlated, but less not correlated.  Finally the free fall time for each
preimage is positively correlated with \tsing, but not much.  

The source of the variance in \tsing\ requires further study.  The lack of
correlation with ``obvious'' parameters is interesting by itself.





